Predicate Abstraction via Symbolic Decision Procedures

We present a new approach for performing predicate abstraction based on symbolic decision procedures. Intuitively, a symbolic decision procedure for a theory takes a set of predicates in the theory and symbolically executes a decision procedure on all the subsets over the set of predicates. The result of the symbolic decision procedure is a shared expression (represented by a directed acyclic graph) that implicitly represents the answer to a predicate abstraction query. We present symbolic decision procedures for the logic of Equality and Uninterpreted Functions (EUF) and Difference logic (DIFF) and show that these procedures run in pseudo-polynomial (rather than exponential) time. We then provide a method to construct symbolic decision procedures for simple mixed theories (including the two theories mentioned above) using an extension of the Nelson-Oppen combination method. We present preliminary evaluation of our Procedure on predicate abstraction benchmarks from device driver verification in SLAM.

==> background.tex <==
\section{Background}

\subsection{Definitions}
Theory, terms, predicates. Inference rules. 



==> inferencerules.tex <==
\begin{figure}[htbp]
\small{
\infrule[Symmetry]
  { X=Y }
  { Y=X }

%\vspace{0.1in}

\infrule[Transitivity]
  { X=Y \andalso Y=Z }
  { X=Z }

%\vspace{0.1in}

\infrule[Contradiction]
  { X=Y \andalso X \not= Y }
  { \bot }

%\vspace{0.1in}

\infrule[Congruence]
  { X_1=Y_1 \andalso \cdots \andalso X_n=Y_n }
  { f(X_1, \cdots, X_n)=f(Y_1, \cdots, Y_n) }

\caption{\label{fig:euf_rules} Inference rules for theory of equality and uninterpreted functions.}
}
\end{figure}


\begin{figure}[htbp]
\tiny{
\infrule[TransLtLeq]
  { X<Z+C \andalso Z \leq Y+D}
  { X<Y+(C+D) }

\vspace{0.1in}

\infrule[TransLeqLt]
  { X \leq Z+C \andalso Z < Y+D}
  { X<Y+(C+D) }

\vspace{0.1in}

\infrule[TransLeqLeq]
  { X \leq Z+C \andalso Z \leq Y+D}
  { X \leq Y+(C+D) }

\vspace{0.1in}

\infrule[ContraLt]
  { X < Y+C \andalso Y \bowtie X+D \andalso C+D \leq 0}
  { \bot }

\vspace{0.1in}

\infrule[ContraLeq]
  { X \leq Y+C \andalso Y \leq X+D \andalso C+D < 0}
  { \bot }

\vspace{0.1in}

\infrule[LeqToEq]
  { X \leq Y \andalso Y \leq X}
  { X = Y }

\caption{\label{fig:diff_rules} Inference rules for Difference logic.}
}
\end{figure}


==> referee_comments <==
%% Please find comments on the reviewers suggestions %%
%% Our comments start with ++ %%

The referee reports:
Referee no 1:

 * This is an excellent paper and can be accepted for Logical Methods
in Computer Science as it is

The main contribution of this paper is that it shows how symbolic
decision procedures (SDPs) may be used to perform predicate
abstraction, i.e., given a set of predicates P and a formula e, they
can compute the weakest boolean formula F_P(e) over P that implies
e. These SDPs may be combined using an extension of the Nelson-Oppen
method to construct SDP for mixed theories. The paper describes
psuedo-polynomial time SDPs for the logic of Equality and
Uninterpreted Functions and the Difference Logic. They also give some
experimental results to consolidate their claim that SDPs are an
efficient technique for computing predicate abstraction.

The main idea behind the paper is that given sets of predicates G and
E for a theory T, the SDP symbolically executes T's decision procedure
on G'\cup{ \neg e | e \in E}, for each subset G' of G. The result of
the execution is a shared expression representing the subsets G' such
that (G' \cup {\neg e | e \in E}) is unsatisfiable. Thus given a set
of predicates P and a boolean formula e which is a disjunction of
predicates in E, the SDP can compute the cover F_P(e) as SDP(P \cup
P~, E) which returns the minterm over P that satisfies e. Using the
results in this paper, this can be then extended to any e in CNF form
and different SDPs may be combined in an Nelson-Oppen style.

The paper is well written and all the key ideas are clearly explained
with the help of examples wherever necessary.

One obvious direction of future work, as noted by the authors
themselves, is to investigate what other theories admit a SDP. Some
such theories may be linear arithmetic, list operations, etc. If
possible, it might help if the authors stated in the paper the
intuition behind deciding what kind of theories are likely to have a
SDP. The implementation section is weak, as pointed out below, and it
would be desirable to see a better comparison with UCLID.

++ We agree with this suggestion of a better comparison with
UCLID. However, the UCLID tool is not actively maintained and it was
hard to translate the SLAM benchmarks used in this paper to the UCLID
format. Beside, the predicate abstraction engine in UCLID uses the
Zchaff SAT solver (from 2001) and it is hard to compare the efficiency
of the two approaches, since both approaches (UCLID based and SDP
based) can be considerably improved with more recent SAT solvers and
better engineering. 

++ We have added a couple of lines in Section 5 stating that based on
the results in the CAV'03 paper, the runtimes appear comparable on the
a similar set of SLAM benchmarks generated in '03, as both of them
finish within a few seconds on most queries.

In my opinion the paper should be accepted for publication because of
the novelty of their approach to predicate abstraction. By using BDDs
as their data-structure, they demonstrate that their technique appears
to be efficient in practice. The problem they are trying to tackle is
quite important and their solution is interesting and credible.





II. Typos

Page 3 : line 5 -- disjunction of *cubes* over the predicates or their
                   negations
Page 3 : line 7 -- *Their* technique requires ...
Page 6 : line 11 -- Each theory has *at* least one ...
Page 10: in proof 2 (b) last line  -- *eval(t[g_j,m-1],G')* = true and
                                      thus *eval(t[g,m], G')* = true Page 12: in Example 2: W terminates --&#62; W stabilizes


++ Fixed

III. Suggestions

Page 4. In syntax of formulas: why not call predicate symbols relation symbols?
This avoids overloading the term "predicate".

++ We have since realized that it would be best to call them
"literals" in the theory. However, we have decided to keep the term
"predicate" since it is used consistently within the paper. 

Page 4 : Figure 1 -- move the definition of formula under that of
atomic-formula.

++ Fixed

Page 5 - Third last paragraph (point 1) - it is not immediately  clear
as to why one cannot introduce auxiliary variables. Explain?

++ This has been explained more clearly.

Page 8 : Figure 4 --
	  (i) Change statement 2(b) to "for all predicates g"
	  2: In the saturation step, it would be a good idea to use
	  the symbol p to denote a predicate instead of g because we
	  generally view g to belong to the set G, while I suppose the
	  authors here want g to represent "any" predicate in theory T
	  - the exposition would become much clearer that way.

++ While that is partly correct, we have used g to be a predicate in
many sets (W, G, W') etc., but is alway bound to a set. We wanted to
use p only for members of P.

	  (ii) You may want to title step 2 as saturation to sync it
	  with the other two steps.

++ Done

IV. Other Comments

* Related Work section - the comparison with [JM05] seems unfair
   because they can use interpolation to compute the set of predicates
   to represent the abstraction of the system from scratch, while in
   this approach the authors need to be seeded with a set of
   predicates P to then compute the predicate cover F_P(e) such that
   F_P(e) => e.


++ In JM05, the predicates have to be still provided. The
technique avoids computing the most precise approximation (F_P)
eagerly and uses interpolants to derive it lazily.

* Implementation section - the comparison with UCLID is not very
   convincing. The one example that is used to compare the approach
   with UCLID may be inherently ill-suited to the way UCLID works -
   one would like to see the comparison of the two tools on an actual
   test case. Also, one interesting experimental result might be to
   use the decision procedure inside SLAM (or some other tool) and
   then report the speed-up observed. The point that SDP's are faster
   than ordinary DP's is driven home fairly well in the discussion
   given in the paper so the comparison result with ZAPATO was sort of
   expected. However, it would be very interesting to see how the
   SPD's help scale up practical software verification tools.

   Further, this technique gives the "most precise" predicate abstraction.
   Is that precision really required in the SLAM examples? If not, the
   comparison is somewhat skewed in favor of the current method. It will
   be better to compare on the examples from JM05 that do need more precise
   abstractions than Cartesian abstraction (the default in SLAM).

++ These are very good suggestions, but we haven't been able to
perform the evaluation of the impact of the improvement of predicate
abstraction on the overall performance. Besides, it is non-trivial
work to add few SLAM specific axioms for memory to the tool. We have
been working on a future work to study the impact.

   However, the 10X improvement is impressive, and the potential of
   the technique is clear.





Referee no 2:

 * The paper can be accepted for Logical Methods in Computer Science after minor revisions.

The paper presents a symbolic technique for computing the weakest
formula over a set of predicates P that implies a target formula
E. Specifically, if E is given as a clause (e_1 || .. || e_n) then the
technique computes the set of all subsets P' of P such that the
conjunction of the elements of P' \cup {!e_1, ..., !e_n} is
unsatisfiable. The overall approach is to compute symbolically (using
BDDs) and incrementally a shared data structure that represents the
desired set of P's. The authors prove that their approach works in
polynomial time for the logic of equality with uninterpreted functions
and in pseudo-polynomial time for difference logic. The paper also
describes a Nelson-Oppen style approach for obtaining a symbolic
decision procedure (SDF) for formulas consisting of symbols from
multiple theories by combining the SDPs for each individual
theory. Finally, the authors present experimental results that show
impressive gains over existing approaches for predicate abstraction.

Overall, the paper is quite well written and I have only some minor
quibbles.

Very early on (e.g., abstract and page 2 line 4) the authors talk
about the satisfiability of a set of formulas. Later on, they clarify
that this means that the formulas are implicitly conjuncted. It would
be helpful to make this clarification up front.

++ Added a line in introduction. 

The authors use a symbol (a dot on top an "=") for definitions and
equalities. It would be nice to explain what this symbol stands for
and why it is used instead of the more standard "=" symbol.

++ We have used \doteq for mostly to define variables and sets. 

Page 5 last sentence: Is the method proposed by McMillan [McM02]
exponential since we are not allowed to introduce auxiliary variables?
If it is exponential then the overall predicate abstraction step also
becomes exponential despite the pseudo-polynomial complexity of your
procedure. Please clarify.

++ That is correct. The bounds are only for the case when e is a
clause. This is mentioned in the last paragraph of Section 2.

Section 3, second line after the inference rule R: "has least one" ==>
"has at least one".

++ Fixed.

Figure 3: Clarify the notation [1,k]. Does it mean a set closed on
both sides, i.e., { x | x >= 1 && x <= k}?

++ Clarified in the figure. 

1st sentence after definition 2: "simply" appears twice. I suggest
dropping the first "simply". Also instead of 'drop "bounded"' you can
say 'drop the term "bounded"'.

++ Done

Para after definition 2: Last two sentences are confusing. I am not
sure how the first of these two sentences is implied by the
second. Also, I thought the second sentence is the definition for
"bounded saturation".

++ If we can establish a finite bound for derivDepth_T(G), then the
saturation-based procedure terminates. Moreover, since DP_T implements
A_T, which is a decision procedure for T, DP_T is a decision procedure
for T.

I was a little confused about why you formulated your SDP procedure in
such a manner till I recalled that E is a clause (e_1 || ... || e_n)
and you want to compute the weakest formula over G that implies E. I
think bringing this connection up early on in Section 3.2 would help
the reader.

++ We say that explicity in the last line of Section 2.

Fig 4 does not mention BDDs and it is not clear how the sharing takes
place. Everything seems explicit. If the sharing is indeed because you
can use a data structure like BDD then it would help to mention this
while you are describing the SDP algorithm.

++ Have mentioned in Page 9, that the output t[e] can be thought of 
as a shared expression or a Boolean circuit. Encoding a circuit into a
BDD is fairly standard.

Same page as Fig 4, second last line: "For any predicate g" ===> "For
any predicate g in W'".

++ We actually mean for any predicate g, since a predicate may not be
in W, but may be derivable in the current step for the first time.

I found the word "derivation" a little overloaded. What is added to
S(g) is not a derivation for g but rather the predicates from which
there is a derivation for g. Alternatively this means that the cube
added to S(g) implies g since the inference rules are sound. Perhaps
it would help to clarify this point.

++ S(g) actually captures the derivation tree for g, where each
derivation step is an instance of a inference rules of the theory. 

Definition 3: What is an "evaluation"? Please define precisely or
refer to an earlier definition.

++ Fixed.


Para after theorem 1, last line: "after i - 1 iterations" ===> should
add the extra condition that "i > 0" for the sake of precision.

++Fixed

Proof of Lemma 1: Case 1: add space between "true" and "for".

++ Fixed

Proof of Lemma 1: What about the reverse implication for the base case
as well as the inductive steps for part 2 of the lemma.

++ We do prove both sides of the implication. We show that g \in W
\implies eval(..) = true, and g \not\in W \implies eval(..) = false. 

++ The way the proof works is that we show eval(...) = true is only
possible when g \in W. 

Proof of Lemma 2: Inductive step. I could not follow case
2(a). Specifically, I don't see how the inductive hypothesis implies
that for every g_j, eval (... g_j ...) is false. This seems too
strong.

++ This is correct. We have corrected to say that there is some g_j,
such that eval(...g_j..) is false. 


Section 5: While the comparison with DP-base methods is impressive, I
would suggest adding more details such as:

- How were the 665 queries selected? Was it done according to some
criterion or randomly?

++ This was the set of benchmarks generated from the regression tests
of the tool.

- Does the 100x speedup occur irrespective of the number of
predicates? If not, a table showing how the speedup varies with the
number of predicates would be helpful.

- Can you give a table showing how many cubes were used by the
DP-based methods even after all the optimizations. Also contrast this
with the number of cubes in the result computed by the SDP
procedure. This might help shed more light on "why" SDP is such a good
idea in practice even though it may be exponential in the worst case.

++ These are very good suggestions, but since the SDV tool has
undergone a lot of changes since the original paper, it is hard to
extract the statistics for the paper. 

Section 5: I thought the comparison with UCLID was a little
contrived. The diamond example seems unrealistic as you yourself argue
in the second para: "However, most problems in practice have a few
cubes ...". Also, since the UCLID experiments were done on a slower
CPU, please clarify if the times in the table of Fig 8 were scaled
accordingly. I would suggest one of three choices: (a) Present
experimental results with UCLID and the same benchmarks you use for
comparison with the SD-based approach; (b) Drop the comparison with
UCLID altogether; (c) Clarify that the comparison with UCLID in its
present form is not very realistic, or, argue why it is still
realistic.

++ We have added some qualitative comparison with uclid based tool in
the result section. 



==> tom_intro.tex <==
\section{Introduction}
\label{sec:intro}

Predicate abstraction is a technique for automatically creating
abstract models of finite and infinite state
systems~\cite{graf-cav97}. Let $E = \{ e_1, \cdots, e_n \}$ be a set
of predicates over the state space of a system. Given another
predicate $e$, the basic problem in predicate abstraction is to find
the weakest boolean function $F_E(e)$ over the predicates $E$ that
implies $e$.  The function $F_E(e)$ may be represented as a
disjunction $c_1 \vee \cdots \vee c_m$, where each $c_j$ (a so-called
``minterm'') is a conjunction of literals $l_{j_1} \wedge \cdots
\wedge l_{j_n}$ such that each $l_{j_k} \in \{ e_k, \neg e_k \}$ and
such that each $c_j$ implies $q$.  The naive approach to compute
$F_E(e)$ is to enumerate each of the $2^n$ minterms and query a
theorem prover to see if the formula $c_j \implies e$ is valid, for
each minterm $c_j$. If so, the minterm $c_j$ is included in $F_E(e)$.
Otherwise, it is not.

The problem of computing $F_E(e)$ appears to be inherently exponential
in $n$ (the number of predicates in $E$).  Various techniques have
been considered for optimizing the predicate abstraction
process~\cite{XYZ}, but all have worst-case behavior $O(2^n)$.  This
is bad because in practice the number of minterms in $F_E(e)$ can be
much smaller than $2^n$. Thus, most techniques end up performing much
wasted work, considering (potentially exponentially many) minterms
that do not imply $e$.

We present a new technique to exploit the sparsity of minterms that
imply $q$ in the universe of all $2^n$ possible minterms over $E$.  We
consider a restricted (and decidable) logic for which we can construct
a data structure in time and space polynomial in $n$ from which we can
output $F_E(e)$ in time proportional to the size of $F_E(e)$, as
measured by the number of minterms in $F_E(e)$.  That is, our
technique is ``output sensitive''. Of course, in the worst case, the
size of $F_E(e)$ may be $O(2^n)$ but when minterms that imply $e$ are
scarse our technique will be dominated by a polynomial bound rather
than an exponential one.

% 1. A Decision procedure takes G and set of facts and a goal g and
% checks is G U {~g} is satisfiable.

%            2. Our procedure takes a set E and g, and
%            "symbolically" simulates the action of a theorem
%            prover to check the satisfiability for any subset E' (E'
%            \subseteq E ) and g. 


To understand our approach, it is instructive to consider what a
decision procedure for a decidable logic $L$ does. Given a set of
predicates $E$ in the logic $L$ and a goal predicate $g$, a decision
procedure $DP_L$ checks whether or not $(\bigwedge_{e \in E} e) \wedge
\neg g$ is satisfiable. The logic $L$ can be characterized by a set of
axioms and inference rules, which $DP_L$ applies to resolve whether or
not the input formula is satisfiable.

Our procedure takes a set of predicates $E$ (in logic $L$) and a goal
predicate $g$ and ``symbolically'' simulates the action of $DP_L$ to
check the satisfiability for every subset $E'$ of $E$ with respect to
$g$. In the process, it constructs an expression to denote all the
possible computations of $DP_L$. With $E$ predicates, we can have
$2^n$ such subsets, and our procedure simulates the behavior of $DP_L$
on each of them. We show that our process works for theories for which
a decision procedure can be constructed using a Nelson-Oppen
combination of other decision procedures. The proof and all the
arguments depend on this observation and is not dependent on whether
the computations are stored explicitly or as a directed acyclic graph
(DAG). For simple theories (equality with uninterpreted functions and
difference constraints), our process builds a compact
(pseudo-polynomial sized) data strucutre that can be effectively
evaluated to produce $F_E(e)$ in time proportional to the size
of $F_E(e)$.
            
This process is analagous to the symbolic simulation of a transition
system with a transition relation and an initial condition.  In our
case, the inference rules of the logic serve as the transition
relation and the set of predicates $E$ and axioms of the logic serve
as the initial state condition. We use the max-derivation depth (which
exists for the given decidable logics) to prove convergence, which is
similar to symbolic simulating until the diameter of the state space
of a system.

%Our technique generates all the derivations of the goal predicate $q$
%from the set of predicates $P$ but maintains a shared DAG (direct
%acyclic graph) representation of the derivations to avoid an
%exponential blowup. We show that this representation has polynomial
%and pseudo-polynomial complexity for equality with interpreted
%functions (EUF) and difference logic (separation constraints of the
%form $x \leq y + c$ (over the integers), respectively. For certain
%mixed theories, we provide a way to construct the shared
%representation of the derivations of the combined theory by modularly
%combining the shared representation of individual theories.

%The shared representation of the derivations can be used for 
%generating compact Shared Boolean programs. We also use an efficient
%way to enumerate the set of derivations (that can be exponential
%in the worst case) by using Binary Decision Diagrams. Since the 
%output of predicate abstraction is usually sparse, the BDD tends to
%remain small for most examples. 

Experimental evaluation of the technique for SLAM. We also extend 
our method to handle non-atomic goals by first converting the goal
to an equivalent CNF expression. 

\comment{
The contributions of the paper:
\begin{itemize}
\item Efficiently represent the derivations for atomic predicates in 
a theory. 
\item For mixed theories with certain restriction, we can use Nelson-Oppen
framework to perform the task modularly. Convergence criteria 
dependent upon particular representation. 
\item Provide two refinements of this technique with complementary
strengths on simple theories. 
\begin{enumerate}
\item With {\bf dag} representation, we can provide a pseudo polynomial
sized shared representation of the derivations. Can also provide
efficient enumeration using BDDs in practice.  
\item With the {\bf worklist} algorithm, we can provide an output
sensitive (?) technique. The technique is {\it incremental}. Suited for
Nelson-Oppen combination and Boolean program construction. 
\end{enumerate}
\item Experimental evaluation
\begin{enumerate}
\item Results on predicate abstraction queries from SLAM. Compare with
Simplify-based method and SAT-based quantification. 
Data with both approaches (size of shared expr, time) etc.
\item Effect on SLAM loop (?). 
\end{enumerate}
\item Extend it to handle queries with Boolean structure. 

\end{itemize}
}

